Cosmology with Phase 1 of the Square Kilometre Array; Red Book 2018: Technical specifications and performance forecasts

We present a detailed overview of the cosmological surveys that will be carried out with Phase 1 of the Square Kilometre Array (SKA1), and the science that they will enable. We highlight three main surveys: a medium-deep continuum weak lensing and low-redshift spectroscopic HI galaxy survey over 5,000 sqdeg; a wide and deep continuum galaxy and HI intensity mapping survey over 20,000 sqdeg from z = 0.35 - 3; and a deep, high-redshift HI intensity mapping survey over 100 sqdeg from z = 3 - 6. Taken together, these surveys will achieve an array of important scientific goals: measuring the equation of state of dark energy out to z ~ 3 with percent-level precision measurements of the cosmic expansion rate; constraining possible deviations from General Relativity on cosmological scales by measuring the growth rate of structure through multiple independent methods; mapping the structure of the Universe on the largest accessible scales, thus constraining fundamental properties such as isotropy, homogeneity, and non-Gaussianity; and measuring the HI density and bias out to z = 6. These surveys will also provide highly complementary clustering and weak lensing measurements that have independent systematic uncertainties to those of optical surveys like LSST and Euclid, leading to a multitude of synergies that can improve constraints significantly beyond what optical or radio surveys can achieve on their own. This document, the 2018 Red Book, provides reference technical specifications, cosmological parameter forecasts, and an overview of relevant systematic effects for the three key surveys, and will be regularly updated by the Cosmology Science Working Group in the run up to start of operations and the Key Science Programme of SKA1.

==> Continuum/Continuum.tex <==
\textit{Contributions from Carlos Bengaly,
Jos\'e Luis Bernal, 
Tamara M.\ Davis,
Matt Jarvis,
Roy Maartens,
David Parkinson, 
Alvise Raccanelli, 
Dominik J.~Schwarz, 
Thilo M.~Siewert (alphabetical for now - on behalf of the SKA Cosmology SWG)}
%an author list scheme similar to what was used in: http://arxiv.org/abs/1606.00180



In this chapter we summarise the cosmological science we expect to extract from the SKA continuum galaxy survey.  The continuum galaxy survey will use all the available extragalactic objects that can be observed by the SKA as cosmological tracers. The aim is to detect as many galaxies as possible, at the expense of not acquiring detailed redshift information for each object.  This has the advantage of allowing us perform a very deep survey quickly by averaging over all frequency data to increase the signal-to-noise in each object's measured flux. This allows continuum radio surveys to rapidly access a much larger volume than the other cosmological surveys. %{\blue Further advantages arise because the synchrotron spectrum of radio emission is a power-law, making $k$-corrections much easier than for optical surveys; and the emission propagation is unaffected by dust obscuration.}

The advantage of tracing out structure through continuum emission also presents some limitations, as the lack of redshift information prevents such surveys being exploited for many powerful cosmological probes (e.g. radial BAO, redshift-space distortions) without external redshift information from the optical or 21cm. The continuum sample therefore maps out the distribution of matter in the Universe in angular space as a function of flux density, rather than the full three-dimensional distribution from a galaxy redshift survey.

The main cosmological science will come from the auto-correlation of these galaxies, and their cross-correlation with other tracers, for example the cosmic microwave background (CMB) or optical galaxies. Auto- and cross-correlations are sensitive to the strength of clustering in the universe, and the effects of gravitational lensing, and thus allow us to test cosmological models (see Sect.~\ref{sect:angcorr}). 
The long, high-redshift tail of continuum galaxy surveys also contains valuable cosmological information.  We can identify this high-redshift tail in our sample by by cross-identifying our sample with lower-redshift optical/near-infrared catalogues, allowing one to identify the low-redshift galaxies, and leaving a large sample in a wide high-redshift bin \citep{Camera:2012ez}.  
Using the SKA, cross-correlation between high-redshift radio sources and low-redshift optical galaxies will allow us to reconstruct the propagation of light by gravitational magnification \citep{Raccanelli2011}. 


There has already been success in detecting the cross-correlation of radio galaxies with the CMB using the continuum galaxy catalogue from the  NRAO VLA Sky Survey \citep[NVSS;][]{1998AJ....115.1693C}.  A correlation between these two samples should be generated by the Integrated Sachs-Wolfe Effect (see Sect.~\ref{sect:isw}), and this was used to detect the effect of the mysterious acceleration of the Universe, driven by the dark energy \citep{BoughnCrittenden,2008PhRvD..77l3520G,2008MNRAS.386.2161R}. 


Finally, the distribution of radio galaxies will allow us to measure  the direction and amplitude of the cosmic dipole (see Sect.~\ref{sect:dipole}), which will be an important test of the fundamental cosmological principle, and provide complimentary information on the nature of the CMB dipole \citep{2015aska.confE..32S}. %[arxiv:1501.03820].

\subsection{Assumed telescope and survey specifications}

%The flux sensitivity for dual-polarisation receivers is given by
%\begin{equation}
%S_{\rm rms} = \frac{2k_BT_{\rm sys}}{A_{\rm eff}N_{\rm dish}\sqrt{2\delta_\nu t_p}} \,,
%\end{equation}
%where $N_{\rm dish}$ and $A_{\rm eff}$ are the number and effective collecting area of the detectors, $\delta_\nu$ is the bandwidth of the observed channel, $T_{\rm sys}$ is the total system temperature, and $t_p$ is the integration time per pointing. Here we assume that the contribution to the total system temperature from the sky is given by $T_{\rm sys} = T_{\rm recv} + T_{\rm sky}$. 

%\textbf{COMMENT BY DOMINIK: THIS DESCRIBES BAND 2, BUT AT LEAST FOR THE WIDE SURVEY WE SHOULD USE BAND 1, WHO IS GOING TO WORK ON THAT?}

For the radio continuum survey design we consider two possible options. 
For the telescope capabilities we follow the specifications given in table 1 of \cite{Bull2016} for the SKA1-MID rebaselined design using Band 2, which covers 950--1760 MHz, and Band 1, which covers 350--1050\,MHz. Our two options both assume a 10,000 hour survey, but aim for different depths and areas:



\begin{enumerate}
\item {\bf Medium-deep:} The first option is a medium-deep survey that covers a 5000 square degree area in Band 2, and would be commensal with the SKA weak lensing shear survey. This would produce high-quality images, most of which would be usable for the continuum angular clustering measurements. The flux limit is estimated to be 8.2$\mu$Jy assuming a 10-sigma rms detection threshold.
\item {\bf Wide:} The second option, a 20,000 square degree wide survey in Band 1, would be a rolling survey conducted with the HI Intensity Mapping survey. This would cover four times the area of the medium-deep survey, to approximately half the depth (since the flux limit scales in inverse proportion to the square root of the integration time, $1/\sqrt{t_p}$).   Given the relative performance of Band 1 vs Band 2 the flux limit is predicted to be slightly more than double the medium-deep survey, at $22\,\mu$Jy assuming a 10-sigma rms detection threshold. One potential limitation of a survey optimised for intensity mapping is that the resolution may be too low to generate a high-fidelity sample of extragalactic point sources, a matter that will be resolved by more detailed simulation of the SKA-MID telescope.

\end{enumerate}

\begin{figure}
\begin{center}
\includegraphics[width=0.95\textwidth]{Continuum/Nz_SKA_MID_B2_5000sqdegs_combined.png}\\
\includegraphics[width=0.95\textwidth]{Continuum/Nz_SKA_MID_B1_20000sqdegs_combined.png}
%\includegraphics[width=0.45\textwidth]{Nz_SKA_MID_B2_5000sqdegs_species.png}
\caption{\label{fig:surveynz} The total number  (\textit{left}) and number  of each galaxy species (\textit{right}) as function of redshift $N(z)$ for a 5000 sq. degree survey (\textit{above}) and a 20000 sq. degree survey (\textit{below}) on SKA1-MID, assuming a flux limit of 8.2$\mu$Jy (for the medium-deep survey, using band 2) and 22.8$\mu$Jy (for the wide survey, using band 1), both assuming 10-sigma detection.  The galaxy types are star forming galaxy (SFG), starburst (SB), Fanoroff-Riley type-I and type-II radio galaxies (FR1 \& FR2), and radio-quiet quasars (RQQ). }
\end{center}
\end{figure}

%\begin{figure}[htp]
%\begin{center}

%\includegraphics[width=0.45\textwidth]{Nz_SKA_MID_B2_20000sqdegs_species.png}
%\caption{\label{fig:20000sqdeg} The total number density and number density of each galaxy species as function of redshift $N(z)$ for the wide 20,000 sq. degree survey, assuming a flux limit of 16.4$\mu$Jy (10-sigma detection).}
%\end{center}
%\end{figure}

 

In figure \ref{fig:surveynz} we plot the expected number distribution as a function of redshift of all radio galaxies (left) and split by galaxy type (right), for the two different surveys. These numbers are generated using the SKA Simulated Skies ($S^3$) simulations\footnote{http://s-cubed.physics.ox.ac.uk/}, based on \cite{Wilman2008}. 


We also need to choose a model for the galaxy bias. Each of the species of source (i.e.\ starburst, star-forming galaxy, FRI-type radio galaxy, etc.) from the $S^3$ simulation has a  different bias model, as described in \cite{Wilman2008}. These models increase bias continuously with redshift, but that will become unphysical at high redshift so here we follow the approach of \cite{Raccanelli2011} holding the bias constant above a cut-off redshift. The bias model we have assumed for the different species as a function of redshift is plotted in figure \ref{fig:bias_model}.  %{\red **How is this actually done?  i.e. How can we hold bias constant above a cut-off redshift if the bias increases continuously with redshift in the simulations?**} 
The true nature of the bias for high-redshift, low luminosity radio galaxies remains currently unknown, and such a cutoff is disputed. \citet{2014MNRAS.442.2511F} point out that a sharp cut-off to the bias is not physical and violates the halo model -- see their figure 2 and discussion below it.  The choice of bias model therefore remains a source of uncertainty, but one that we will be able to resolve with the SKA. 
\begin{figure}[htp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Continuum/continuum_bias_model.png}
\caption{\label{fig:bias_model}Bias as a function of redshift for the different  source types, as
following the simulated $S^3$ catalogues of \cite{Wilman2008}.}
\end{center}
\end{figure}


Finally, we will be able to divide our sample into redshift bins, based on photometric or statistical information. While these bins will not be as accurate as spectroscopic redshifts, they will still allow us to recover some of the 3D information from the distribution of galaxies. The assumed redshift bin distribution is given in table \ref{tab:contredshiftbins}. As well as predicting the number and bias of the galaxies for the two strategies, we also use the fluxes from the $S^3$ simulation to predict values for the slope of the source-flux to number density power law, which couples the observed number density to the magnification (magnification bias), given by
\begin{equation}
\alpha(S) = -\frac{\partial\log N_0(S)}{\partial \log S}\,,
\end{equation} 
where $S$ is the flux and $N_0$ is the unmagnified number density power law \citep{Bartelmann:2001}. Magnification bias arises because faint objects are more likely to be seen if they are magnified by dense lines of sight.  This changes the clustering properties of the sample, and thus contains cosmological information.  Magnification bias depends on the slope of the flux vs number density power-law, because it depends on the number of faint galaxies that are available to get magnified into observability. As the relative number of bright objects changes with redshift, we also expect the slope of the power law to be redshift dependent.

\begin{table}[htp]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
Bin & $z_{\rm min}$ & $z_{\rm max}$ &\multicolumn{3}{|c|}{Wide survey}  &\multicolumn{3}{|c|}{Medium-deep survey} \\
 &  &  & Num  ($\times 10^6$) &  bias & power-law slope &Num  ($\times 10^6$) &  bias & power-law slope  \\ \hline
0 & 0.000  & 0.300  & 16.48  &  0.890 & 0.838  & 8.27  & 0.864  & 0.760 \\
1 & 0.300 & 0.600  &  21.60  &  1.018 &  1.211 &12.50  & 0.947  & 1.038\\
2 & 0.600 & 0.900  &  28.28  &  1.265 &  1.212 & 16.12  & 1.176 &  1.054\\
3 & 0.900 & 1.200  &  24.48  &  1.465 &   1.351 & 15.55  & 1.345 &  1.186\\
4 & 1.200 & 1.500  &  23.80  &  2.132 &   1.375  & 15.70 &  1.820  & 1.298\\
5 & 1.500 & 1.800  &  16.60  &  2.124 &   1.330 & 11.54  & 1.857  & 1.221\\
6 & 1.800 & 2.100  &  12.16  &  2.519 &   1.574 & 90.80  & 2.056  & 1.462\\
7 & 2.100 & 3.000  &  19.96  &  3.228 &  1.284 & 15.79 &  2.769 &  1.246\\
8 & 3.000 & 6.000  &  12.92  &  3.859 &  1.122 & 12.24  & 3.350  & 1.247 \\ \hline
\end{tabular}
\caption{\label{tab:contredshiftbins} For each proposed redshift bin we present the redshift range, number of galaxies, galaxy bias, and magnification bias, for the two survey strategies.  The bias refers to the number-weighted average of the bias of all galaxies in the bin. }
\end{table}

\subsection{Forecasting}
\label{sec:cosmologyobs}

To estimate the effectiveness of the surveys and make predictions for the constraints on the cosmological parameters, we simulate the auto- and cross-correlation galaxy clustering angular power spectra, including the effects of cosmic magnification and the Integrated Sachs-Wolfe effect (ISW). In the case of galaxy clustering and ISW, we limit the analysis to the multipoles $\ell_{\rm min}\leq \ell\leq 200$, where $\ell_{\rm min} = \pi/(2f_{\rm sky})$ and $f_{\rm sky}$ is the fraction of sky surveyed.

\subsubsection{Angular Correlation Function}\label{sect:angcorr}

The two-point distribution of radio galaxy positions in angle space can be represented by the  angular correlation power spectrum $C_{\ell}$, which is given by
\begin{equation}
\label{eqn:cl}
  C_{\ell} = \langle a_{\ell m}^g a_{\ell m}^{g*}\rangle = 4\pi \int \frac{dk}{k} \Delta^2(k)[ W_\ell^g(k)]^2\,,
\end{equation}
where $\ell$ is the multipole number, $k$ is the wavenumber,  $\Delta^2(k)$ is the logarithmic matter power spectrum and $W^g_{\ell}(k)$ is the radio galaxy window function. This form assumes a single redshift bin with the galaxies distributed across this bin to give some window function \citep[e.g.][]{2008PhRvD..77l3520G,2008MNRAS.386.2161R},
\begin{equation}
\label{eqn:wincl}
  W_\ell^g(k) = \int \frac{dN(\chi)}{d\chi} b(z)D(z)j_\ell[k\chi]d\chi\,.
\end{equation}
Here $dN/d\chi$ is distribution of sources per steradian with comoving radial distance $\chi(z)$ within the redshift bin (brighter than some survey magnitude or flux limit), $b(z)$ is the bias factor relating tracer overdensity to matter overdensity, $D(z)$ is the growth factor of density perturbations, and $j_\ell(x)$ is the spherical Bessel function.

This statistic encodes the density distribution projected on to the sphere of the sky, and so smooths over structure along the line of sight. This can dampen the effect of redshift-space distortions on the angular power spectrum (which we have neglected from Eq.~\ref{eqn:wincl}) for broad redshift distributions, but these can become important as the distributions narrow \citep{Padmanabhan2007}. 

When two non-overlapping redshift bins are considered, the window functions should be entirely separate, and the cross-correlation of density perturbations between these two bins measured through $C_{\ell}^{i,j}$ (given by equation \ref{eqn:cl}) should be negligible. However, the observed galaxy distribution is also affected by gravitational lensing, which can induce a correlation between the two bins, creating an observed correlation between the positions of some high redshift galaxies and the distribution of matter at low redshift. Although in most cases negligible, gravitational lensing also affects galaxy autocorrelations.

Gravitational lensing has two effects on the light bundle, a shearing effect on the image shape, and magnification of image size (though surface brightness is conserved); in addition, the volume that we observed behind the lensed is also affected. At some position on the sky $\vec{\theta}$ there is some unlensed set of sources with number density $N_0(m)dm$, within a magnitude range $[m,m+dm]$. The effect of gravitational lensing will mean that the number of sources we actually observe will be $N(m,\vec{\theta})dm$, given by \citep{Broadhurst:1994qu}
\begin{equation}
  N(m,\vec{\theta})dm=\mu^{\alpha(m)-1}N_0(m)dm\,,
\end{equation}
where $\alpha$ is the slope of the magnitude-number power law, and $\mu$ is magnification, which in the weak lensing limit, is given by  the convergence $\kappa$, by $\mu(\vec{\theta}) \simeq 1 + 2\kappa(\vec{\theta})$.

The convergence is related to the matter overdensity along the line of sight \citep{Bartelmann:2001} by
\begin{equation}
  \kappa(\vec{\theta}) = \frac{3\Omega_m H_0^2}{2} \int_0^{\chi_H}  g(\chi)d_A(\chi) \frac{\delta(d_A\vec{\theta},\chi)} {a(\chi)} d\chi\,,
\end{equation}
where $\chi_H$ is the horizon distance,  $d_A(\chi)$ is the angular diameter  distance, $a$ is the scale factor and $g(\chi)$ is a lensing window function, giving the lensing efficiency along the line of sight,
\begin{equation}
  g(\chi)=\int_\chi^{\chi_H} d\chi'N_\chi(\chi')\frac{d_A(\chi'-\chi)}{d_A(\chi')}\,,
\end{equation}
for which $N_\chi(\chi)d\chi$ is the source redshift distribution.  These integrals extend to the horizon distance because we are calculating how many faint galaxies beyond the lens will be magnified into our observable sample.

As only the observed galaxy distributions (which are affected by gravitational lensing) can be measured, it is impossible to measure the galaxy angular power spectrum decoupled from magnification. Hence, the observed angular power spectrum is obtained by the correlation of density and magnification perturbations:
\begin{equation}
C_\ell = C_\ell^{\rm gg} + C_\ell^{\rm g\mu} + C_\ell^{\rm g\mu} +C_\ell^{\rm \mu\mu} 
\end{equation}

The dominant term in which magnification is involved is the cross-correlation between the high redshift sources and the low redshift lenses, given by 
\begin{equation}
\label{eqn:cl_lens}
  C_{\ell}^{g\mu} = \langle a_{\ell m}^g a_{\ell m}^{\mu}\rangle = 4\pi \int \frac{dk}{k} \Delta^2(k)W_\ell^g(k) W_{\ell}^\mu\,.
\end{equation}

Each entry of the Fisher matrix of the observed galaxy clustering (i.e., including magnification effects) is given by:
\begin{equation}
F_{\alpha\beta} = \sum_\ell \frac{\partial \vec{C_\ell}}{\partial\alpha}{\rm Cov}^{-1}\frac{\partial \vec{C_\ell}}{\partial\beta},
\end{equation}
where $\alpha$ and $\beta$ are two cosmological parameters of interest, $\vec{C_\ell}$ is a vector composed of all possible cross correlations $C_\ell^{\rm (ij)}$, (i and j being redshift bin, with j$\geq$i) and the covariance is computed from the errors in the power spectra. Assuming Gaussianity, the covariance is given by i.e. \cite{2016JCAP...05..009R}:
\begin{equation}
{\rm Cov}_{\rm \left[(ij),(pq)\right]} = \frac{\tilde{C}_\ell^{\rm ip}\tilde{C}_\ell^{\rm jq}+\tilde{C}_\ell^{\rm iq}\tilde{C}_\ell^{\rm jp}}{(2\ell+1)f_{\rm sky}}, \quad\quad \tilde{C}_\ell^{\rm ij} = C_\ell^{\rm ij}+\frac{\delta_{\rm ij}}{dN(z_{\rm i})/d\Omega}.
\label{eq:Fisher_gg}
\end{equation}
In this expression, q$\geq$p are also redshift bins, $dN(z_{\rm i})/d\Omega$ is the average number of sources per steradian (to account for the shot noise) and $f_{\rm sky}$ is the fraction of the sky observed by the survey. Using Equation \ref{eq:Fisher_gg} ensures that the full covariance is accounted for properly, which is especially important in the case of overlapping bins.

%The error on the cross-correlation power spectrum of radio background with optical foreground sources is given by
%\begin{equation}
%  \sigma_{C_{\ell}^{g\mu}} = \sqrt{\frac{C^2_{g\mu}+(C_g^b+C_{\rm shot}^b)(C_g^f+C_{\rm shot}^f)}{(2\ell+1)f_{\rm sky}}}
%\end{equation}
%where $f$ and $b$ refer to the foreground (lenses) and background sources (objects), and ``shot'' stands for the shot noise.

%The shot noise definition is given as \citep{ZhangPen2006}
%\begin{equation}
%C^b_{\rm shot} = 4\pi f_{\rm sky}[1 +N^b_{\rm noise}/N_b]/N_b \,.
%\end{equation}
%The extra factor $1 +N^b_{\rm noise}/N_b$ accounts for the contaminations of false peaks in the selected background sample. These false peaks does not correlate with each other, so their only effect is to increase the shot noise.

\subsubsection{Integrated Sachs Wolfe Effect}\label{sect:isw}

The distribution of matter in the Universe can also be measured by the effect on the CMB temperature anisotropies, through the Integrated Sachs-Wolfe effect (ISW). The redshifting and blueshifting of CMB photons by the intervening gravitational potentials generates an apparent change in temperature, given by
\begin{equation}
  \label{eqn:ISW}
  \left(\frac{\Delta T}{T}\right)_{\rm ISW}(\mathbf{x}_0,\mathbf{n}) = 2 \int_{\eta_{\rm dec}}^{\eta_0} \dot\Phi(x_0-\mathbf{n}(\eta-\eta_0),\eta) d\eta\,.
\end{equation}
Here $\dot\Phi$ is the time-derivative of the lensing potential $(\Phi+\Psi)/2$ (assuming no anisotropic stress), with respect to conformal time $\eta$, $\mathbf{x_0}$ is the observer's position (the photon position at time $\eta_0$), and $\mathbf{n}$ is the photon trajectory. In this way the CMB photons are influenced by the gravitational evolution of the post-recombination Universe.

Since the distribution of matter (which generates the gravitational potentials) can be mapped through the distribution of tracer particles, such as galaxies,  the effect is detected by cross-correlating the positions of galaxies and temperature anisotropies on the sky. The cross-correlation power spectrum between the galaxies (at low-redshift) and the temperature anisotropies is given by
\begin{equation}
  C_{\ell}^{gT} = \langle a_{\ell m}^g a_{\ell m}^T\rangle =4\pi\int \frac{dk}{k} \Delta^2(k) W^g_{\ell}(k)W^T_{\ell}(k) \,,
\end{equation}
where $\Delta^2(k)$ is the logarithmic matter power spectrum and $W^g_{\ell}(k)$ and $W^T_{\ell}(k)$ are the window functions for the radio sources and CMB respectively. We can use the equation for the temperature anisotropies (eqn.~\ref{eqn:ISW}) to determine $W^T_{\ell}(k)$ through linear theory.



\subsubsection{Cosmic dipole}\label{sect:dipole}

The prediction of the established standard model of cosmology is that the radio sky should be isotropic on large scales. Deviations from isotropy are expected to arise from proper motion of the Solar system with respect to the isotropic CMB (the cosmic dipole), the formation of large scale structures and light propagation effects like gravitational lensing. 

%The cosmic dipole has already been detected in the CMB,  which is commonly assumed to be caused by the proper motion of the Sun with respect to the cosmic heat bath at $T_0 = 2.7$ K. 
The CMB dipole is commonly assumed to be caused by the proper motion of the Sun with respect to the cosmic heat bath at $T_0 = 2.725$ K 
%The CMB dipole 
and was measured by Planck with high accuracy. This allows us to infer a proper motion of the Sun with a speed of $v = (369.0 \pm 0.9)$ km/s towards the galactic coordinates $l = (264.00 \pm 0.03)$ deg and $b = (48.24\pm 0.02)$ deg \citep{Planck2016I,Planck2016VIII}. However, the CMB dipole could also contain other contributions, e.g.\ a primordial temperature dipole or an integrated Sachs-Wolfe (ISW) effect. In the Planck best-fit $\Lambda$ cold dark matter cosmology ($\Lambda$CDM) both effects are expected to be sub-dominant, but one has to keep in mind that the cosmic variance of the dipole is huge and thus the primordial temperature and the ISW dipoles remain unknown.

It is thus %interesting and 
of fundamental importance to test the proper motion hypothesis. The extragalactic radio sky offers an excellent opportunity to perform an independent test of this hypothesis. %In $\Lambda$CDM 
It is expected that the radio dipole is dominated by the kinematic dipole. 
%similar to the CMB. 
This is not the case for galaxy surveys at visible or infrared wavebands, as the number counts in those wavebands in wide area surveys are %typically 
dominated by objects at redshifts well below unity. In contrast, radio continuum surveys have median redshifts well above one. Current estimates of the radio dipole show good agreement with the CMB dipole direction, but find a dipole amplitude that is a factor of 2 to 5 larger than expected \citep{2002Natur.416..150B, 2011ApJ...742L..23S, 2013A&A...555A.117R, 2017MNRAS.471.1045C, 2017arXiv171008804B}. 

We estimate the ability of SKA continuum surveys to measure the cosmic radio dipole, by means of mock catalogues that include the effects of large scale structure and the kinematic dipole. Details of that study will be published elsewhere. The mock catalogues were produced assuming the Planck best-fit flat $\Lambda$CDM model~\citep{2016A&A...594A..13P} %as the fiducial cosmology 
and so we computed the angular power spectrum via {\sc CAMB sources}~\citep{2011PhRvD..84d3516C}. The assumed redshift distribution $dN/dz$ is shown in Fig.~\ref{fig:surveynz}, the $b(z)$ follows~\cite{2015ApJ...814..145A}.
%We fix the maximum multipole as $\ell=128$, and 
The available sky area is $f_{sky} \simeq 0.52$ due to the removal of the galactic plane on low galactic latitudes ($|b| \leq 10^{\circ}$). Using this prescription, we produced ensembles of $100$ catalogues each, using the lognormal code {\sc flask}~\citep{2016MNRAS.459.3693X}, so the radio source positions are distributed following its expected clustering, as well as its shot noise. %For each mock we produce a set of HEALPix maps at Nside = 64 and at various flux thresholds. 
We also produce mocks in which the effect of the local structure is suppressed by assuming that we will be able to remove the local structure by means of optical or infra-red catalogues, or by means of the HI redshift measured by the SKA for the low-redshift sources. The effect of the kinetic dipole is implemented by boosting the maps of galaxy number densities according to the theoretical expectation \citep{1984MNRAS.206..377E}, 
\begin{equation}
\left[\frac{\mathrm{d} N}{\mathrm{d}\Omega} (S, \mathbf{n})\right]_{\mathrm{obs}} = \left[\frac{\mathrm{d} N}{\mathrm{d}\Omega} (S, \mathbf{n})\right]_{\mathrm{rest}} \left( 1 + [2 + x (1+\alpha)] \frac{\mathbf{n}\cdot\mathbf{v}} {c}\right),
\end{equation}
where $S$ denotes the flux density threshold of the survey, $\mathbf{n}$ the direction on the sky and $\mathbf{v}$ the Sun's proper motion. This expression assumes that radio sources follow a power-law spectral energy distribution, $S \propto \nu^{-\alpha}$ with $\alpha = 0.75$. %is the assumed mean spectral index of radio sources. 
The source counts are assumed to scale with $S$ as $\mathrm{d} N/\mathrm{d}\Omega \propto S^{-x}$, and we assume $x = 1$. The values of $\alpha$ and $x$ are chosen in agreement with current measurements. %The true values at SKA fluxes densities might turn out to be different. 
Our assumptions result in an expected kinematic radio dipole amplitude of $A = 0.0046$ pointing to the CMB dipole direction.  

We estimate the radio dipole direction and amplitude of the generated mock catalogues by means of a quadratic estimator in pixel space on a HEALPix\footnote{HEALPix package \url{http://healpix.sourceforge.net/}} grid with Nside = 64. 
%to find the best fitting dipole direction and amplitude. In doing so 
We also vary the monopole, but do not include higher multipole moments. The advantage of using pixel space is that incomplete sky coverage does not bias the results.

\subsection{Results}

In order to explore the potential of the radio continuum surveys of SKA on cosmology, we study the following extensions to $\Lambda$CDM: a model with an equation of state that varies with time, namely $(w_0w_a)$CDM following the CPL parametrization introduced in \cite{CPL_w0wa}; a model with deviations from General Relativity, parametrized as scale independent modifications to the ratio of the graviational potentials and their relation with the energy density, $\Lambda$CDM+$\mu_0$+$\gamma_0$ \citep{2013MNRAS.429.2249S,Baker_mgclass}; a model in which the spatial sector of the Universe is not forced to be flat, $\Lambda$CDM+$\Omega_k$; and a model  with deviations from Gaussian initial conditions in the local limit (parametrized with $f_{\rm NL}$), $\Lambda$CDM+$f_{\rm NL}$. In all these cases, we assume a $\Lambda$CDM model with the mean values from the temperature and polarization power spectra (PlanckTTTEEE+lowP) from Planck Collaboration as our fiducial cosmology: $\Omega_{\rm b}h^2 = 0.02225$, $\Omega_{\rm cdm}h^2=0.1198$, $h=0.6727$, $\log (10^{10}A_s)=3.094$ and $\sum m_\nu=0.06$ eV. We use the public Boltzmann code CLASS \citep{Lesgourgues:2011re} to compute the theoretical observables. 
 We also show our predicted constraints on the cosmic dipole.





\subsubsection{Results - time varying dark energy}
A common extension to $\Lambda$CDM is to model dark energy as a scalar field. We use the CPL parametrization to model this effect as a variation of the equation of state of dark energy with time \citep{CPL_w0wa}:
\begin{equation}
w(a) = w_0+(1-a)w_a.
\end{equation}
We show the predicted 68\% and 95\% confidence level constraints on the deviation of the dark energy parameters $w_0$ and $w_a$ from $\Lambda$CDM for the wide and medium deep surveys in red Figure \ref{fig:Gaussian_bins_w0wa}. We also show the current constraints from Planck TTTEEE+lowP and BAO observations \citep{2016A&A...594A..13P}\footnote{MCMC chains and covariance matrices publicly available in \href{http://pla.esac.esa.int/pla/}{http://pla.esac.esa.int/pla/}.} in blue and the combination of both in black. Marginalized 68\% confidence level predicted constraints on the deviations can be found in Table \ref{tab:cont-big}.
\begin{figure}[htp]
\begin{center}
\includegraphics[width=0.9\textwidth]{Continuum/w0wa_forecast_gg.pdf}\\
\includegraphics[width=0.9\textwidth]{Continuum/MG_forecast_gg.pdf}
\caption{\label{fig:Gaussian_bins_w0wa}68\% and 95\% confidence level forecast constraints on the deviation of the dark energy parameters $w_0,w_a$ (top) and modified gravty parameters $\mu_0,\gamma_0$ from their fiducial values for the wide (left) and medium-deep (right) surveys, using galaxy clustering data, including the effects of cosmic magnification. We show Planck+BAO constraints in blue,  SKA forecasts in red and the constraints for the combination of both experiments in black. We show here that for the dark energy medium-deep survey adds very little to the existing constraints, while the wide survey effectively halves the error bars. }
\end{center}
\end{figure}




%\begin{table}
%\centering
%\begin{tabular}{|l|l|c|c|c|c|c|c|} \hline
% &   &\multicolumn{6}{|c|}{Parameters}   \\
% &  & \multicolumn{2}{|c|}{Galaxy Clustering (GC)} & \multicolumn{2}{|c|}{GC+ISW} & \multicolumn{2}{|c|}{GC+ISW+Planck} \\
%Survey &  Model &  $w_0$  & $w_a$  & $w_0$  & $w_a$ &  $w_0$  & $w_a$  \\ \hline
%Wide & $(w_0w_a)$CDM & 0.15  & 0.38  & 0.15  & 0.38 & 0.072 & 0.19\\
%Med-Deep & $(w_0w_a)$CDM &  0.30 & 0.78  & 0.30 & 0.78  & 0.19& 0.48\\ \hline
%\end{tabular}
%\caption{\label{tab:cont-DE}68\% confidence level predicted constraints on deviations of the evolving dark energy parameters $w_0$ and $w_a$ from the fiducial values from continuum galaxy clustering measurements from the two survey strategies.}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|} \hline
& &\multicolumn{6}{|c|}{Data combination and parameters} \\
Survey& Model & \multicolumn{2}{|c|}{Galaxy Clustering (GC)} & \multicolumn{2}{|c|}{GC+ISW} & \multicolumn{2}{|c|}{GC+ISW+Planck} \\ \hline
& & \hspace{5mm} $w_0$\hspace{5mm} & \hspace{5mm}$w_a$\hspace{5mm} & \hspace{5mm}$w_0$\hspace{5mm} & \hspace{5mm}$w_a$\hspace{5mm} & \hspace{5mm}$w_0$\hspace{5mm} & \hspace{5mm}$w_a$\hspace{5mm} \\ \hline
Wide & $(w_0w_a)$CDM & 0.14 & 0.37 & 0.14 & 0.37 & 0.065 & 0.18\\
Med-Deep & $(w_0w_a)$CDM & 0.30 & 0.78 & 0.30 & 0.78 & 0.19& 0.48\\ \hline \hline
& & $\mu_0$ & $\gamma_0$ & $\mu_0$ & $\gamma_0$& $\mu_0$ & $\gamma_0$ \\ \hline
{Wide} & $\Lambda$CDM+$\mu_0$+$\gamma_0$ & 0.23 & 0.69 & 0.18& 0.42  & 0.065 & 0.16 \\
{Med-Deep} & $\Lambda$CDM+$\mu_0$+$\gamma_0$ & 0.42 & 1.2 & 0.33& 0.83  & 0.094 & 0.24 \\
\hline\hline
& & \multicolumn{2}{|c|}{$\Omega_k$} & \multicolumn{2}{|c|}{$\Omega_k$} & \multicolumn{2}{|c|}{$\Omega_k$} \\ \hline
Wide & $\Lambda$CDM+$\Omega_k$ & \multicolumn{2}{|c|}{$7.2\times 10^{-3}$}  & \multicolumn{2}{|c|}{$7.2\times 10^{-3}$} & \multicolumn{2}{|c|}{$9.0\times 10^{-4}$}\\
Med-Deep & $\Lambda$CDM+$\Omega_k$ & \multicolumn{2}{|c|}{$4.6\times 10^{-3}$} & \multicolumn{2}{|c|}{$4.6\times 10^{-3}$} &\multicolumn{2}{|c|}{$1.8\times 10^{-3}$}\\ \hline\hline
& & \multicolumn{2}{|c|}{$f_{\rm NL}$} & \multicolumn{2}{|c|}{$f_{\rm NL}$} & \multicolumn{2}{|c|}{$f_{\rm NL}$} \\ \hline
Wide & $\Lambda$CDM+$f_{\rm NL}$ & \multicolumn{2}{|c|}{1.4 }  & \multicolumn{2}{|c|}{1.4} & \multicolumn{2}{|c|}{1.3}\\
Med-Deep & $\Lambda$CDM+$f_{\rm NL}$ & \multicolumn{2}{|c|}{4.4 } & \multicolumn{2}{|c|}{4.4 } &\multicolumn{2}{|c|}{3.3}\\ \hline
\end{tabular}
\caption{\label{tab:cont-big} Predicted constraints from continuum galaxy clustering measurements using the two different survey strategies (wide and med-deep). These are 68\% confidence levels on each of the parameters of the four different cosmological models we tested. The three main columns show results of galaxy clustering by itself (left), galaxy clustering combined with Integrated Sachs Wolfe constraints (centre), and when Planck priors are added to GC+ISW (right).}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Results - modified gravity}
Deviations from GR can be encoded by the following effective description of the relation between the metric potentials:
\begin{equation}
-2k^2\Psi=8\pi G_Na^2\rho D\mu(a,k),
\end{equation}
\begin{equation}
\frac{\Phi}{\Psi} = \gamma(a,k),
\end{equation}
where the GR limit is $\mu=\gamma=1$. We consider scale independent deviations from GR which emerge at late times (we neglect the effect at $z>5$), hence we assume they are proportional to the dark energy density parameter:
\begin{equation}
\mu(a,k) = 1+\mu_0\frac{\Omega_\Lambda(a)}{\Omega_{\Lambda,0}}, \qquad \gamma(a,k) = 1+\gamma_0\frac{\Omega_\Lambda(a)}{\Omega_{\Lambda,0}}.
\end{equation}
Therefore, we include $\mu_0$ and $\gamma_0$ as free parameters in our analysis. We use the public modification of CLASS, MGCLASS\footnote{\url{https://gitlab.com/philbull/mgclass}} \citep{Baker_mgclass} to compute the cosmological observables including modified gravity. 68\% confidence level predicted constraints on the deviations of these parameters from the GR limit for the two survey strategies are shown in table \ref{tab:cont-big}. As in the case of the $(w_0w_a)$CDM model, we also show the predicted 68\% and 95\% confidence level constraints on the modified gravity parameters for the wide and medium deep surveys in red Figure \ref{fig:Gaussian_bins_w0wa}. 
We include the combination of SKA forecasts and current constraints from Planck TTTEEE + lowP and BAO and RSD observations \citep{Planck_DE-MG} in black. As the Planck Markov chains for these models are not public, we use the marginalized 68\% confidence level constraints reported in \cite{Planck_DE-MG} (and therefore we do not show the corresponding individual constraints in Figure \ref{fig:Gaussian_bins_w0wa}.)
%\begin{table}[htp]
%\centering
%\begin{tabular}{|l|l|c|c|c|c|c|c|} \hline
% &   &\multicolumn{6}{|c|}{Parameters}   \\
% &  & \multicolumn{2}{|c|}{Galaxy Clustering (GC)} & \multicolumn{2}{|c|}{GC+ISW} & \multicolumn{2}{|c|}{GC+ISW+Planck} \\
%Survey &  Model &  $\mu_0$  & $\gamma_0$ &  $\mu_0$  & $\gamma_0$&  $\mu_0$  & $\gamma_0$ \\ \hline
%{Wide} & $\Lambda$CDM+$\mu_0$+$\gamma_0$ & 0.24  & 0.72  & 0.18& 0.44    & 0.065  & 0.17  \\
%{Med-Deep} & $\Lambda$CDM+$\mu_0$+$\gamma_0$ & 0.42  & 1.2  & 0.33& 0.83    & 0.094  & 0.24  \\
% \hline
%\end{tabular}
%\caption{\label{tab:cont-MG}68\% confidence level predicted constraints on the modified gravity parameters $\mu_0$ and $\gamma_0$ with respect to their GR limit from continuum galaxy clustering measurements from the two survey strategies.}
%\end{table}


\subsubsection{Results - curvature}
We show the predicted marginalized 68\% confidence level constraints on the deviation from flatness parametrized by $\Omega_k$ (assuming a $\Lambda$CDM+$\Omega_k$ model)  for the wide and medium deep surveys in Table \ref{tab:cont-big}. 

%\begin{table}[htp]
%\centering
%\begin{tabular}{|l|l|c|c|c|} \hline
% &   &\multicolumn{3}{|c|}{Parameters}   \\
% &  & Galaxy Clustering (GC) & GC+ISW & GC+ISW+Planck \\
%Survey &  Model &  $\Omega_k$ & $\Omega_k$ & $\Omega_k$ \\ \hline
%Wide & $\Lambda$CDM+$\Omega_k$ &  $2.6\times 10^{-3}$     & $2.6\times 10^{-3}$  &  $1.5\times 10^{-3}$\\ 
% Med-Deep & $\Lambda$CDM+$\Omega_k$ &  $4.6\times 10^{-3}$  &  $4.6\times 10^{-3}$   &$1.8\times 10^{-3}$\\ \hline
% \end{tabular}
%\caption{\label{tab:cont-curvature}68\% confidence level predicted constraints on deviations from flatness ($\Omega_k=0$) from continuum galaxy clustering measurements from the two survey strategies.}
%\end{table}

\subsubsection{Results - non-Gaussianity}

The very largest-scale modes of the matter spectrum can be measured through all-sky surveys, and since these modes will have remained outside the horizon since the hot big bang, they will preserve any imprint of primordial non-linearities in the generation of structure. These non-linearities are manifested as non-Gaussianities in the distribution of amplitudes, and can be parameterized through the local non-Gaussianity parameter, defined in terms of the amplitude of the quadratic contributions to the metric potential $\Phi$ as a local function of a single Gaussian field $\phi$,
\begin{equation}
\Phi(x) = \phi(x) + f_{\rm NL}\left(\phi^2(x)-\langle\phi^2\rangle\right) + \ldots\,,
\end{equation}
though this is not the only type of non-Gaussianity that can be generated. Predicted constraints on $f_{\rm NL}$ from the two survey configurations can be found in table \ref{tab:cont-big}. For other forms of non-Gaussianity, and the predicted constraints from SKA-like surveys, see \cite{Raccanelli2017}. 

%\begin{table}[htp]
%\centering
%\begin{tabular}{|l|l|c|c|c|} \hline
% &   &\multicolumn{3}{|c|}{Parameters}   \\
% &  & Galaxy Clustering (GC) & GC+ISW & GC+ISW+Planck \\
%Survey &  Model &  $f_{\rm NL}$ & $f_{\rm NL}$ & $f_{\rm NL}$ \\ \hline
%Wide & $\Lambda$CDM+$f_{\rm NL}$ &  1.6     & 1.6  &  1.5\\ 
% Med-Deep & $\Lambda$CDM+$f_{\rm NL}$ &  4.4  &  4.4   &3.3\\ \hline
% \end{tabular}
%\caption{\label{tab:cont-NG}68\% confidence level predicted constraints on the local non-Gaussianity parameter $f_{\rm NL}$ from continuum galaxy clustering measurements from the two survey strategies.}
%\end{table}
We find the constraints on $f_{\rm NL}$ from the medium-survey to be not significantly better than those currently made by the Planck surveyor, $f_{\rm NL} = 2.5 \pm 5.7$ \citep{PlanckNG2016}. In contrast the wide survey will improve on this constraint by more than a factor of three.

A deeper survey, such as the medium-deep survey described here, may be able to provide more competitive constraints on $f_{\rm NL}$  through the use of different radio galaxy populations as tracers of different
mass halos, as described in \cite{2014MNRAS.442.2511F}. We leave a detailed analysis of such a use of these surveys for the future.



\subsubsection{Results - Cosmic dipole}

\begin{figure}[htp]
\centerline{
\includegraphics[scale=0.45]{Continuum/ska_Ns64_mockmap.png}}
\caption{Simulated source count per pixel for the SKA-MID wide area survey at a central frequency of 700 MHz and a flux threshold of $22.4 \mu$Jy in galactic coordinates and Mollweide projection at HEALPix resolution  $N_{\rm side}=64$ including the kinematic dipole and cosmic structure up to multipole moment $\ell_{\rm max}=128$.}
\label{mock_example}
\end{figure}

\begin{figure}[htp]
\centerline{
\includegraphics[width=0.65\linewidth]{Continuum/Dipoles_22muJy_a.pdf}
\includegraphics[width=0.35\linewidth]{Continuum/Amplitudes_22muJy_a.pdf}}
\caption{Dipole directions (left) and histogram of dipole amplitudes (right) based on 100 large scale structure simulations each for a flux density threshold of $22.4 \mu$Jy at 700 MHz without kinetic dipole (pink), with kinetic dipole (purple) and with the contribution from the local structure dipole removed (red). The blue dot shows the direction of the CMB dipole. The results are displayed in galactic coordinates and in stereographic projection.}
\label{dipole_direction22}
\end{figure}

%\begin{figure}
%\centerline{
%\includegraphics[width=0.9\linewidth]{Amplitudes_22muJy.pdf}}
%\caption{Histogram of the dipole amplitude estimates based on 100 large scale structure simulations for a flux density threshold of $22.4 \mu$Jy at 700 MHz without kinetic dipole (pink), with kinetic dipole (purple) and with the contribution from the local structure dipole removed (red).}
%\label{dipole_amplitude22}
%\end{figure}

Fig.~\ref{mock_example} shows an example of the simulated skies for a flux density threshold of $22.4 \mu$Jy at a central frequency of $700$ MHz (Band 1). The results from a set of $100$ such simulations is shown in Fig.~\ref{dipole_direction22}. The large scale structure contributes a dipole with a mean amplitude of $A = 0.0031 \pm 0.0016$. This prediction depends on the assumed luminosity functions, spectral energy distributions, bias, redshift and luminosity evolution of radio sources,
%and is thus model dependent, 
see e.g.\ \cite{2016JCAP...03..062T}. Identifying radio source morphology and the broad frequency coverage of the wide survey will help us to better constrain those unknowns and improve the prediction for the structure dipole. Fig.~\ref{dipole_direction22} also shows the expected total radio dipole, which obtains contributions from large scale structure and the proper motion of the solar system. The expected kinematic contribution dominates the structure contribution and the measured amplitude is $A = 0.0056 \pm 0.0017$ in direction $(l,b) = (263.5\pm 28.0, 38.8\pm 19.7)$ deg.
%from our 100 simulations. 
One sees that the expected total dipole direction is centered on the CMB dipole direction, but with some scatter due to the large scale structure. 

The structure dipole is in fact dominated by contributions from local structure. When we remove the low-redshift structure dipole ($z < 0.5$) we measure the dipole direction $(l,b) = (265.3 \pm 4.9, 46.4 \pm 4.3)$ deg in excellent agreement with the CMB dipole direction and we extract an amplitude of $A = 0.0047 \pm 0.0004$, in excellent agreement with the expected $A = 0.0046$. The distributions of dipole amplitudes from the set of $100$ simulations is shown in the right panel of Fig.~\ref{dipole_direction22}.

We also simulated catalogues with $S = 5, 10$ and $16 \mu$Jy, which show that the structure dipole depends on the flux density threshold, providing an extra handle to separate them from the kinematic dipole. %Details of that analysis will be presented elsewhere.  
In none of our simulations was shot noise a limitation, in contrast to contemporary  radio continuum surveys \citep{2015aska.confE..32S}. 



\subsection{Summary}

When exploring the extensions to $\Lambda$CDM considered here, the wide survey forecasts predict a much better performance regarding the constraining power on these extra parameters than the medium-deep survey. This is not surprising as modifications related to the dark energy or modified gravity generate the most pronounced differences in the cosmological observables at low redshifts. In addition, observational signatures from the non-Gaussianity of primordial structure or the large-scale homogeneous curvature of the Universe arise at very large scales. Therefore, the medium-deep survey, while being more precise at large redshift, is less competitive for cosmology than the wide survey. The wide survey is able to access larger scales and more density-field modes than the deep survey, giving smaller errors on the observables and better measurement of the parameters, even taking into account cosmic variance. %Moreover, the cosmic variance can be partially removed with multitracing techniques.

Measurement of the cosmic radio dipole with an SKA-MID wide survey in band 1 will be possible at a significantly higher precision than has previous been possible, and thus truly test the nature of the CMB dipole. That survey can be done in parallel to the HI intensity mapping effort and actually benefit from HI redshifts to local sources. The kinematic and local structure dipole can be separated by means of identifying the low-redshift sources and splitting the source catalogue accordingly.

\section*{Acknowledgements}
Some of the results in this work have been derived using the HEALPix \citep{2005ApJ...622..759G} package.




==> HI_gal/HI_gal.tex <==
\FloatBarrier

This survey mode involves detecting the redshifted 21cm emission from many individual galaxies above the confusion limit, predominantly at low redshift ($z \lesssim 0.4$). At a minimum, the positions and spectroscopic redshifts of the detected galaxies will be available. The 21cm line widths and angular sizes of some subset of the galaxies can also be measured, allowing direct estimates of peculiar velocities to be made via the Tully-Fisher relation and Doppler magnification effects respectively.

The galaxies detected in this survey mode will not necessarily be well-resolved, but resolved detections can be used to study galaxy dynamics. The variation of the HI content of galaxies over cosmic time is also an important observable for studies of galaxy formation and evolution. All galaxies with a detectable 21cm line are expected to have strong continuum detections, and so this survey is expected to be carried out commensally with a continuum galaxy survey. In fact, characterising the continuum emission along the line of sight to HI-detected galaxies may be necessary to o.

%--------------------------------------------------------------------------
\subsection{Assumed telescope and survey specifications}
%--------------------------------------------------------------------------

For a cosmological HI galaxy survey, we assume a fiducial survey area of $\sim$5,000 deg$^2$, which will be sample variance-limited out to $z_{\rm max} \sim 0.4$, if we assume a 10,000 hr total survey time using Band 2. This would be significantly oversampled (i.e. $n(z) P(k) \gg 1$) at $z\lesssim 0.2$, which provides an opportunity for multi-tracer studies (in which the uncertainty on certain cosmological quantities is dominated by shot noise rather than sample variance). Band 1 is expected to yield too few galaxies for a cosmological survey.

Basic predictions for the number density (and corresponding bias) of galaxies that will be detected by a blind SKA1 HI galaxy survey were made in \cite{2015MNRAS.450.2251Y} for the original SKA1 specifications, and \cite{Camera:2014bwa} provided a sister fitting function for the estimated magnification bias. These calculations were based on the S$^3$-SAX simulations, and assumed that any galaxy with an integrated line flux above a given SNR threshold would be detectable. This paper also includes fitting functions that can be used to rescale the number density and bias for different instrumental specifications.

Updated number density and bias predictions for the current (rebaselined) SKA1 specification were presented in \cite{Bull2016}, and are reproduced in Table~\ref{tab:dndzfits}, using the following fitting functions:
\begin{eqnarray} \label{eq:hi_dndz}
\frac{dN}{dz} &=& 10^{c_1} z^{c_2} \exp({-c_3 z}) ~~~ [{\rm deg}^{-2}]; ~~~~ b(z) = c_4 \exp({c_5 z}).
\end{eqnarray}
This paper included a survey optimisation study to establish the optimal survey area as a function of total survey time. A wide and shallow survey would optimise the survey volume that is sample variance limited. A 5,000 deg$^2$ survey (10,000 hr) would provide a reasonable tradeoff between total volume and maximum redshift.

Alternative number density predictions were made in \cite{2017arXiv170408278H}, using a Bayesian line-fitting method on simulated spectra for continuum-selected galaxies (i.e. a non-blind survey). The population of galaxies that is selected by this method is quite different to those selected using the SNR threshold of \cite{2015MNRAS.450.2251Y} but, coincidentally, the predicted number density curves are very similar. Typically $\sim 10\%$ of continuum galaxies (for a 5,000 deg$^2$, 10,000 hr survey) will have significant detections of the 21cm line using this method.

\paragraph{Impact of RFI:} Bright RFI from navigation satellites is expected to severely impact our ability to detect HI galaxies in the redshift range from approximately $0.09 \lesssim z \lesssim 0.23$, corresponding to $1164-1300$ MHz. Terrestrial RFI is also expected to be present elsewhere in the band, but at a much lower level thanks to the excellent radio-quietness of the SKA1-MID site. Source detection algorithms can incorporate features to reject RFI, such as preferentially selecting double-peaked lines that are characteristic of HI galaxies.

\begin{table}[h]
\centering
{\renewcommand{\arraystretch}{1.6}
\begin{tabular}{|l|r|rrr|rr|r|r|}
%\multicolumn{1}{r|}{Fiducial $k_\mu = $} & \multicolumn{2}{c|}{$0.005$ Mpc$^{-1}$} & \multicolumn{2}{c|}{$0.01$ Mpc$^{-1}$} & \multicolumn{2}{c|}{$0.05$ Mpc$^{-1}$} \\
\hline
{\bf Survey} & \multicolumn{1}{c|}{\bf Thres.} & \multicolumn{1}{c}{$c_1$} & \multicolumn{1}{c}{$c_2$} & \multicolumn{1}{c|}{$c_3$} & \multicolumn{1}{c}{$c_4$} & \multicolumn{1}{c|}{$c_5$} & \multicolumn{1}{c|}{$z_{\rm max}$} & \multicolumn{1}{c|}{$N_{\rm gal} / 10^6$} \\
% * <alkistispou@gmail.com> 2018-03-17T10:00:21.430Z:
%
% ^.
\hline
\multirow{2}{*}{SKA1 B2 Rebase. + MeerKAT} & $5\sigma$~~ & 5.450 & 1.310 & 14.394 & 0.616 & 1.017 & 0.391 & 3.49~~~ \\
 & $8\sigma$~~ & 4.939 & 1.027 & 14.125 & 0.913 & -0.153 & 0.329 & 2.04~~~ \\
\hline
\multirow{2}{*}{SKA1 B2 Alt. + MeerKAT} & $5\sigma$~~ & 5.431 & 1.297 & 14.260 & 0.616 & 1.018 & 0.391 & 3.54~~~ \\
 & $8\sigma$~~ & 4.935 & 1.024 & 14.089 & 0.907 & -0.089 & 0.329 & 2.05~~~ \\
\hline
\end{tabular} }
\caption{Fitting coefficients for $dN/dz$ and $b(z)$ for the SKA HI galaxy surveys, for various detection thresholds (assuming $S_{\rm area} =$ 5,000 deg$^2$). $z_{\rm max}$ is the maximum redshift at which $n(z) P(k_{\rm NL}) > 1$, where $k_{\rm NL}$ is the non-linear scale.}
\label{tab:dndzfits}
\end{table}

\begin{table*}
\centering
\scalebox{0.8}{\begin{tabular}{|ll|r|r|r|r|r|r|r|r|c|c|c|c|c|}
\hline 
\multirow{2}{*}{\bf Telescope array} & & $T_\mathrm{recv}$ & $A_\mathrm{eff}$~ & $D_\mathrm{dish}$ & \multirow{2}{*}{$N_\mathrm{d} \times N_\mathrm{b}$~} & ${\rm FOV}$~ & $\nu_{\rm ref}$~~ & $\nu_\mathrm{min}$~ & $\nu_\mathrm{max}$~ & \multirow{2}{*}{$z_\mathrm{min}$} & \multirow{2}{*}{$z_\mathrm{max}$} & $S_{\rm area}$ IM & $S_{\rm area}$ GS \\
 & & [K]~~ & [m$^2$] & [m]~~ & & [deg$^2$] & [MHz] & [MHz] & [MHz] & &  & [deg$^2$] & [deg$^2$] \\
\hline
\multirow{2}{*}{SKA1-LOW}
 & Rebaselined & 40~~~ & 925~ & 35~~~~ & $455\times3$ & 28~~~~~ & 110~~ & 50~~ & 350~ & 3.06 & 27.4 & \multirow{2}{*}{1,000} & \multirow{2}{*}{---} \\
 & Alternative & 40~~~ & 925~ & 35~~~~ & $455\times3$ & 28~~~~~ & 110~~ & 50~~ & 500~ & 1.84 & 27.4 & & \\
\hline
\multirow{2}{*}{SKA1-MID B1}
 & Rebaselined & 23~~~ & 133~ & 15~~~~ & $130\times1$ & 1.78 & 700~~ & 350~~ & 1050~ & 0.35 & 3.06 & \multirow{3}{*}{25,000} & \multirow{3}{*}{---} \\
 & Alternative & 12~~~ & 133~ & 15~~~~ & $130\times1$ & 1.78 & 700~~ & 450~~ & 825~ & 0.72 & 2.16 & & \\
MeerKAT & UHF-band & 23~~~ & 115~ & 13.5~ & $64\times1$ & 2.20 & 700~~ & 580~~ & 1015~ & 0.40 & 1.45 & & \\
\hline
\multirow{2}{*}{SKA1-MID B2}
 & Rebaselined & 15.5 & 150~ & 15~~~~ & $130\times1$ & 0.87 & 1000~~ & 950~~ & 1760~ & 0.00 & 0.49 & \multirow{3}{*}{25,000} & \multirow{3}{*}{5,000} \\
 & Alternative & 15.5 & 150~ & 15~~~~ & $130\times1$ & 0.87 & 1000~~ & 795~~ & 1470~ & 0.00 & 0.79 & & \\
MeerKAT & L-band & 30~~~ & 122~ & 13.5~ & $64\times1$ & 1.08 & 1000~~ & 900~~ & 1670~ & 0.00 & 0.58 & & \\
\hline
SKA2 & & 15~~~ & 6~ & 3.1~ & $70000\times1$ & 30~~~~~ & 1000~~ & 470~~ & 1290~ & 0.10 & 2.00 & --- & 30,000 \\
\hline
\end{tabular}}
\vspace{0.1in}
\caption{Representative instrumental parameters for various assumed SKA Phase 1 and 2 array configurations and bands. $A_{\rm eff}$ is the effective area per dish or receiving element, and the ${\rm FOV}$ is calculated at the reference frequency, $\nu_{\rm ref}$. $\nu_{\rm min, max}$ are the band edges, and $z_{\rm min, max}$ the corresponding minimum/maximum accessible redshifts. Representative survey areas for intensity mapping (IM) and galaxy surveys (GS) are given in the final two columns. Other quantities are defined in the text.}
\label{tab:skaarrays}
\end{table*}

%--------------------------------------------------------------------------
\subsection{Forecasts}
%--------------------------------------------------------------------------

More information can be extracted from the HI galaxy survey besides the 3D clustering of galaxies. Several additional probes will be supported, as discussed below. These will require alternative analysis pipelines, able to measure marked correlation functions, galaxy sizes, and 21cm line widths. These probes will not drive the survey optimization, but will need to be accommodated in the specifications (e.g. output channel bandwidth).

%--------------------------------------------------------------------------
\subsubsection{Baryon acoustic oscillations and redshift-space distortions}
%--------------------------------------------------------------------------
The baryon acoustic oscillation (BAO) feature is a preferred scale in the clustering of galaxies, set by sound waves emitted in the early Universe when photons and baryons were coupled. Since the true physical scale of the BAO is known from CMB observations, we can use the feature as a `standard ruler' to measure the cosmological expansion rate and distance-redshift relation. This is achieved by separately measuring the apparent size of the BAO feature in the transverse and radial directions on the sky, and comparing with its known physical size (set by the size of the comoving sound horizon during the baryon drag epoch, $r_s(z_d)$). The radial BAO scale is sensitive to the expansion rate, $H(z)$, while the transverse BAO scale is sensitive to the angular diameter distance, $D_A(z)$.

\begin{figure}[t]
 \centering
 \includegraphics[width=0.49\columnwidth]{HI_gal/mg-Hz.pdf}
 \includegraphics[width=0.49\columnwidth]{HI_gal/mg-fsig8.pdf}
 \caption{Forecast constraints on the cosmic expansion rate, $H$, (left panel) and linear growth rate of large-scale structure, $f\sigma_8$, (right panel) for several different experiments, taken from \cite{Bull2016}. A 5,000 deg$^2$, 10,000 hour SKA HI galaxy redshift survey is shown in light blue.}
 \label{fig:hi-forecast} 
\end{figure}

SKA1 will be able to detect and measure the BAO feature at low redshift. This measurement has already been performed by optical spectroscopic experiments, such as BOSS and WiggleZ, but over different redshift ranges and patches of the sky. An SKA1 HI galaxy redshift survey will add an independent data point at low redshifts, $z \sim 0.3$, which will help to better constrain the time evolution of the energy density of the various components of the Universe -- particularly dark energy, which may have an equation of state, $w = P / \rho$, that differs from the value of $-1$ that would be expected if it is simply a cosmological constant. The expected constraints on $H(z)$ and $D_A(z)$ are shown in Fig.~\ref{fig:hi-forecast}, and are typically a few percent. While this is not competitive with the precision of forthcoming optical/near-IR spectroscopic surveys such as DESI and Euclid, it will be at lower redshift than these experiments can access, and so is essentially complementary to them.

Other features that are present in the clustering pattern of galaxies include redshift-space distortions (RSDs), a characteristic squashing of the 2D correlation function caused by the peculiar motions of the galaxies. Galaxies with a component of motion in the radial direction have their spectral line emission Doppler shifted, making them appear closer or further away than they actually are according to their observed redshifts. This results in an anisotropic clustering pattern as seen in redshift space. The degree of anisotropy is controlled by several factors, including the linear growth rate of structure, $f(z)$, and the clustering bias of the galaxies with respect to the underlying cold dark matter distribution, $b(z)$. The growth rate in particular is valuable for testing alternative theories of gravity, which tend to enhance or suppress galaxy peculiar velocities with respect to the GR prediction. RSDs occur on smaller scales than the BAO feature, but can also be detected by an HI galaxy redshift survey as long as the shot noise level is sufficiently low. The nominal SKA1 HI survey will be able to measure the linear growth rate scaled by the normalisation of the matter power spectrum, $f\sigma_8$, to $\sim 3\%$ at $z \approx 0.3$ (see the right panel of Fig.~\ref{fig:hi-forecast}). This is roughly in line with what can be achieved by existing optical experiments in a similar redshift range. While it will provide a useful independent data point, this measurement is not competitive on its own.

%--------------------------------------------------------------------------
\subsubsection{Constraints on modified gravity theories}
%--------------------------------------------------------------------------
As discussed above, measurements of the growth rate allow us to constrain possible deviations from General Relativity over large distance scales. We can convert these measurements into more directly meaningful constraints on the effective strength of gravity, as experienced by the large-scale structure as it collapses. This is often parametrised as a redshift-dependent rescaling of the gravitational constant that appears in the linear growth equation, $G_N \to \mu(z) G_N$. Fig.~\ref{fig:mgparams} shows the constraints on $\mu_0$ that will be achievable with growth rate measurements from RSDs in the nominal SKA1 HI galaxy redshift survey, along with some other standard cosmological parameters and the modified gravity-related parameter $\eta_0$ (which scales the effective gravitational constant seen by light, rather than collapsing matter structures). The constraints are very weak, offering little improvement over existing measurements from the Planck CMB satellite. As such, the alternative methods for testing gravity discussed below are more promising for SKA1.

\begin{figure}[t]
\centering
%\includegraphics[width=0.9\textwidth]{HI_gal/mg_params_planck.png}
\includegraphics[width=0.8\textwidth]{HI_gal/skahi_mg.png}
\caption{\label{fig:mgparams} Forecast constraints on phenomenological modified gravity parameters using the broadband shape of the power spectrum, detected using an SKA1 HI galaxy survey. Planck constraints are included for comparison. The improvement from adding SKA1 is negligible in this particular parametrisation.}
\end{figure}


%--------------------------------------------------------------------------
\subsubsection{Doppler magnification}
%--------------------------------------------------------------------------
\begin{figure}[t]
\centering
%\includegraphics[width=0.9\textwidth]{HI_gal/mg_params_planck.png}
\includegraphics[width=0.7\textwidth]{HI_gal/doppler_mag_snr.pdf}
\caption{\label{fig:doppmag} The signal-to-noise ratio of the Doppler magnification dipole for SKA1 as a function of separation $d$ at $z=0.15$ (the redshift bin in which the SNR is largest). A pixel size of 4 Mpc/h has been assumed. The upper bound and lower bounds are for convergence errors (size noise) of $\sigma_\kappa=0.3$ and $\sigma_\kappa=0.8$ respectively.}
\end{figure}

There is a contribution to the apparent magnification of galaxies due to their peculiar motion, as well as due to weak gravitational lensing. The motion of the galaxies causes a shift in their apparent radial position (as seen in redshift space), while their angular size depends only on the actual (real space) angular diameter distance. As such, a galaxy that is moving away from us will maintain fixed angular size while appearing to be further away than it really is (and thus `bigger' than it should be for a galaxy at that apparent distance). This effect has been called Doppler magnification, and dominates the weak lensing convergence at low redshift \citep{2014MNRAS.443.1900B, 2017MNRAS.471.3899B, 2017MNRAS.472.3936B,Raccanelli:2016avd,Abramo:2017xnp}. It can be detected statistically through the dipolar pattern it introduces in the density-convergence cross-correlation, $\langle \kappa \delta_g \rangle$. The galaxy density, $\delta_g$, can be measured using a spectroscopic galaxy survey like an HI galaxy redshift survey, while the convergence can be estimated from the angular size of galaxies.

As discussed above, an SKA1 HI galaxy redshift survey will yield high number densities of galaxies with spectroscopic redshifts at $z \lesssim 0.4$, approximately covering the redshift range where Doppler magnification dominates the weak lensing convergence. If the HI-emitting galaxies can be resolved, their sizes can also be measured (e.g. from their surface brightness profile in continuum emission), making it possible to measure the Doppler magnification signal using a single survey. Galaxy size estimators often suffer from large scatter, and it remains an open question how well SKA1 will be able to measure sizes. This scatter has a significant effect on the expected SNR of the Doppler magnification signal.

Following the forecasting methodology of \cite{2017MNRAS.472.3936B}, we expect SKA1 to achieve a signal-to-noise ratio of $\sim 8$ on the Doppler magnification dipole for galaxies separated by $\sim 100$ $h^{-1}$Mpc (Fig.~\ref{fig:doppmag}), assuming a size scatter of $\sigma_\kappa = 0.3$ (which is comparable to what optical surveys can achieve).

%--------------------------------------------------------------------------
\subsubsection{Direct peculiar velocity measurements}
%--------------------------------------------------------------------------

The Tully-Fisher relation can be used to infer the intrinsic luminosity of a galaxy from its 21cm line width (a proxy for its rotational velocity). Combined with the measured redshift of the line, this is sufficient to measure the peculiar velocity of the galaxy. Various statistics of the peculiar velocity field can then be used to measure different combinations of cosmological quantities from the 3D density field. We do not currently have forecasts for an SKA1 Tully-Fisher survey but refer the reader to \cite{2014MNRAS.445.4267K} for a set of forecasts that include SKA precursor experiments.

%--------------------------------------------------------------------------
\subsubsection{Void statistics}
%--------------------------------------------------------------------------

Future large-area galaxy surveys will offer an unprecedented spectroscopic view of both large and small scales in the cosmic web of structure. Thanks to its high galaxy density and low bias, the SKA1 HI galaxy survey will allow probing unusually small voids and comoving scales. 

The number counts \citep{Pisani:2015jha, Sahlen:2015wpc}, shapes \citep{Massara:2015msa}, redshift-space distortions \citep{Sutter:2014oca}, and lensing properties \citep{Spolyar:2013maa} of voids are examples of sensitive void probes of cosmological parameters. Voids are particularly sensitive to the normalization and shape of the matter power spectrum, its growth rate, and the effects of screened theories of gravity which exhibit a modification to General Relativity in low-density environments \citep{Voivodic:2016kog}. This is because void distributions contain objects ranging from the linear to the non-linear regime, across scale, density and redshift \citep{Sahlen:2016kzx}. 

\begin{figure}[t]
\centering
\includegraphics[trim={13.2cm 0.3cm 0cm 0.3cm},clip,width=0.5\textwidth]{HI_gal/skarb_voids.pdf}
\caption{\label{fig:voidw0wa} Forecast marginalized parameter constraints for $w_0$ and $w_a$ from SKA1-MID-B2 void counts (gray), {\it Planck}+lensing+BAO (blue), and both combined (yellow). Apart from the cosmological parameters, we have also marginalized over uncertainty in void radius and cluster mass \citep{Sahlen:2016kzx}, and in the theoretical void distribution function \citep{Pisani:2015jha}.}
\end{figure}

\begin{table}[htp]
\vspace{-5pt}
\caption{Forecast dark energy constraints for void counts.}
\label{tab:voidw0wa}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Survey & $\sigma(w_0)$ & $\sigma(w_a)$ & FoM \\
\hline
SKA1-MID-B2 void counts & $0.22$ & $1.84$ & 9 \\
{\it Planck}+lensing+BAO & $0.30$ & $0.85$ & 13 \\
Joint & $0.07$ & $0.34$  & 84 \\ 
\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\end{table}%

We forecast cosmological parameter constraints from the SKA1-MID-B2 HI galaxy survey in our fiducial cosmology, using the Fisher-matrix method. The void distribution is modeled following \citep{Sahlen:2015wpc, Sahlen:2016kzx} using an approximate modeling scheme to incorporate the effects of massive neutrinos on the void and cluster distributions. We also take into account the galaxy density and bias for the survey \citep{Santos:2015dsa}. Below $z \approx 0.18$, the survey is limited by the void-in-cloud limit. Voids smaller than this limit tend to disappear due to collapse of the overdensity cloud within which they are situated.

We expect about $4 \times 10^4$ voids larger than $10\,h^{-1}$ Mpc. The marginalized constraints on $w_0$ and $w_a$ are shown in Fig.~\ref{fig:voidw0wa} and Table~\ref{tab:voidw0wa}. We note that the SKA1 void counts and {\it Planck}+lensing+BAO offer similar but complementary constraining power, and that their combination can strengthen the Figure of Merit by a factor $\sim 6-10$. Including also the sum of neutrino masses as a free parameter only marginally weakens the void constraints. Recalling that additional cosmological information is also available in e.g. shapes/profiles, voids are a promising new probe with the SKA. 

%--------------------------------------------------------------------------
\subsubsection{Astrophysical contamination of cosmological constraints}
%--------------------------------------------------------------------------
The astrophysics acts as an effective `systematic' when placing cosmological and fundamental physics constraints using redshifted 21 cm line studies. The combination of current astrophysical uncertainties on the neutral hydrogen density and bias parameter, $\Omega_{\rm HI}$ and $b_{\rm HI}$ can be shown to lead to about 60\% - 100\% uncertainty in the HI power spectrum \citep{hptrcar2015}. To explore the implications of this effect for future surveys with the SKA, we need to realistically model the astrophysics associated with HI-bearing systems so as to comprehensively assess the impact of the current uncertainties. In \citet{hpar2017, hparaa2017}, this is done by building a data-driven, halo model framework that takes into account the available HI observations (21 cm galaxy surveys, intensity mapping observations, and Damped Lyman Alpha (DLA) systems) across redshifts 0--5 in the post-reionization universe. Such a framework allows an easy integration of the astrophysical uncertainties into forecasts for current and future HI experiments [Padmanabhan, Refregier and Amara, in preparation], and thus provides an understanding of the `astrophysical degradation' expected in recovering cosmological parameters, which is found to be alleviated by the addition of information from multiple tomographic bins.

% \begin{figure}
%  \centering
%  \includegraphics[width=0.49\columnwidth]{HI_gal/ska1gs-zmax.pdf}
%  \includegraphics[width=0.49\columnwidth]{HI_gal/ska1gs-vol.pdf}
%  \caption{The maximum survey redshift and corresponding comoving survey volume, $V_{\rm sur}(0 \!\le\! z \!\le\! z_{\rm max})$, in Gpc$^3$, as a function of survey time and survey area, for an SKA1-MID Band 2 HI galaxy survey in the `Alternative' configuration. The fiducial survey time/area assumed in this study is shown as a red cross. We have assumed that the minimum frequency, $\nu_{\rm min}$, can be adjusted without changing other specifications, and use a detection threshold of $5\sigma$.}
%  \label{fig:hi-optimisation} 
% \end{figure}


% \begin{figure}
%  \centering
%  \includegraphics[width=0.49\columnwidth]{HI_gal/Band_2_snr_B.png}
%  \includegraphics[width=0.49\columnwidth]{HI_gal/Band_2_zhist.png}
%  \caption{From Harrison/Lochner. {\it Right panel:} Number of galaxies expected to be detected per square degree, as a function of redshift. ${\rm SNR}_{\rm vel}$ is the same SNR statistic used by {\bf Yahya}, while $\ln(B)$ is the Bayesian evidence ratio between 21cm line model and the null hypothesis (a flat spectrum with thermal noise).}
%  \label{fig:hi-detection} 
% \end{figure}

\begin{table}[t]
\begin{center}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c|ccr|}
\cline{2-6}
 & \multicolumn{2}{c|}{} & \multicolumn{3}{c|}{\bf SKA1-MID B2 + MeerKAT} \\
\cline{2-6}
 & $z_{\rm min}$ & $z_{\rm max}$ & $n(z)$ [Mpc$^{-3}$] & $b(z)$ & $S_{\rm rms}$ $[\mu{\rm Jy}]$ \\
\cline{1-6}
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Rebase. / Alt.}}} & 0.0 & 0.1 & $2.73 \times 10^{-2}$ & 0.657 & 117.9~~~~ \\
 & 0.1 & 0.2 & $4.93 \times 10^{-3}$ & 0.714 & 109.6~~~~ \\
 & 0.2 & 0.3 & $9.49 \times 10^{-4}$ & 0.789 & 102.9~~~~ \\
 & 0.3 & 0.4 & $2.23 \times 10^{-4}$ & 0.876 & 97.5~~~~ \\
 & 0.4 & 0.5 & $6.44 \times 10^{-5}$ & 0.966 & 93.1~~~~ \\
\cline{1-6}
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Alt.}}} & 0.5 & 0.6 & $1.70 \times 10^{-5}$ & 1.059 & 89.4~~~~ \\
 & 0.6 & 0.7 & $1.72 \times 10^{-6}$ & 1.208 & 106.2~~~~ \\
\cline{1-6}
\end{tabular}}
\caption{Binned number density and bias of HI galaxies, and corresponding flux sensitivity, for SKA1-MID Band 2, assuming a 5,000 deg$^2$, 10,000 hour survey. The detection threshold is 5$\sigma$.} \vspace{-2em}
\label{tab:nzska1}
\end{center}
\end{table}

\FloatBarrier

==> Synergies/synergies.tex <==
\vspace{-0.1in}
\textit{Contributors: D. Bacon, D. Bertacca, S. Camera, S. Cunnington, J. Fonseca, I. Harrison, R. Maartens, A. Pourtsidou, M. Santos.}

\vspace{0.1in}\noindent With next-generation cosmological surveys we are able to map out the large scale structure of the observable Universe. In other words we are able to completely determine with great precision the spatial distribution of matter from scales of hundred-Mpc out to the cosmological horizon and from the present epoch out to the highest observable redshift, reaching  the dark ages of structure formation. The study of the cosmic large-scale structure will allow us to answer two the fundamental issues of the contemporary cosmology: i)  The physical mechanism that generated the inflationary expansion in the early Universe and ii) it general relativity is hold on the largest scales.

Up to now in cosmology the greatest effort has been made to extract statistical information from the distribution of a large number of objects such as galaxies and galaxy clusters. Often errors in cosmological parameters are dominated by statistical errors, which can be reduced by increasing the number of objects. However  precision cosmology will be limited by systematic errors and cosmic variance, rather than statistical errors.  
Complementarity and synergy between the Square Kilometre Array and future survey projects in other wavelengths, i.e. the cosmic microwave background, optical/infrared and X-ray, substantially will reduce systematic errors and cosmic variance (rather than statistical errors) which will become the limiting factors to advance cosmology further.

Here, we summarise and discuss  how complementarity and synergy will be very powerful to tackle major cosmological problems such as dark energy, modified gravity and primordial non-Gaussianity.

\subsection{Radio-optical cosmic shear cross-correlations}
The usual techniques for the measurement of galaxy shapes are based on measurement of galaxy images, as they were developed for optical surveys. However radio interferometers are not able to provide directly images of the observed sky because they measure visibility data instead, precisely the Fourier transform of the sky image at sampled points in the Fourier (uv) domain.

A more natural approach for radio weak lensing is to measure source shapes directly in the visibility domain, avoiding image reconstruction and reducing original data manipulation, i.e systematics introduced by the imaging process.  In \cite{Rivi:2016ccv} they presented an adaptation to radio observations of {\em lens}fit~\cite{Miller:2012am}, an algorithm for shear measurement for optical weak lensing surveys. This version of the method, called RadioLensfit, works  directly in the visibility domain,  and fits a galaxy model computed analytically as the Fourier transform of a S\'{e}rsic exponential brightness profile. They demonstrated that galaxy shape measurement provides acceptably accurate values and additive bias comparable to the requirements on a 5000 $\deg^2$ SKA1 survey for $\textrm{SNR}>18$. 

%Harrison - WL forecasts
In \cite{Harrison:2016stv}, the authors constructed forecasts for cosmological parameter estimation. They shown that the first phase of the SKA (SKA1) could be competitive with experiments such as the Dark Energy Survey (DES), and that the full SKA (SKA2) could potentially provide a  tighter constraint from weak lensing alone than optical cosmic shear surveys, for example  Large Synoptic Survey Telescope (LSST) or a \euclid satellite.

Moreover, as also discussed in \S~\ref{ssec:wl-xcorr}, radio-optical cross-correlations for cosmic shear have another, major advantage with respect to singe-wavelength measurements. Indeed, multi-wavelength cosmic shear analyses are free from additive systematic effects, and they can be used to mitigate the impact of shear calibration errors \cite{Camera:2016owj}. For instance, Fig.~\ref{fig:sys_add} shows the impact of additive residual systematics to the reconstruction of dark energy equation-of-state parameters, $\{w_0,w_a\}$. Left(right) panels refer to Stage III(IV) DETF cosmic shear experiments, with radio, optical/near-IR and their cross-correlation respectively in blue, red and green. The black cross indicates \lcdm. The green solid, correctly centred ellipse shows the unbiased result obtained with the cross-correlation of optical/near-IR and radio surveys (insensitive to additive systematics), whereas dashed, dot-dashed and dotted ellipses are for the residual systematic power spectrum.
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Synergies/Ellipses_w0wa-Add0-eps-converted-to}
    \caption{Marginal joint 1$\sigma$ error contours in the dark energy equation-of-state parameter plane. The black cross indicates the \lcdm\ fiducial values for dark energy parameters. Blue, red and green ellipses are for radio and optical/near-IR surveys and their cross-correlation, respectively. (Details in the text.)}\label{fig:sys_add}
\end{figure*}

%\subsection{Principal component analysis}

%Gong-bo Zhao

%%%%%Text provided by D. Bertacca, but no results from Gong-bo ever arrived, so this subsection should be removed.
%The dark energy and gravity parameters can be constrained  bu using the Principal Component Analysis (PCA) approach used by \cite{Zhao:2008bn, Zhao:2015wqa}. Employing  the PCA, it is possible to forecast the future constraint on the equation of state $w(z)$ of dark energy, and on the effective Newton constant  $\mu(k,z)$  and the gravitational slip, $\gamma(k,z)$, which parameterise (in first approximation)  the effects of modified gravity.

\subsection{Synergies for primordial non-Gaussianity and relativistic effects}
%e.g. work of Fonseca, Camera, Santos \&  Maartens 
The  understanding of the Universe  on very-large scales is one of the major science topics for the SKA. 
The SKA will be able to probe a vast volume and represents a crucial instrument for studying  the properties of the Universe on the largest cosmic scales and is in a crucial position to change this state of art and push forward the study 
The two main observables on ultra-large scales are fundamental for understanding the properties of the Universe: the primordial non-Gaussianity (PNG) and horizon-scale general relativistic and projection corrections (GR). 

The best current constraints on PNG are from the Planck CMB experiment, but future CMB experiments are unlikely to improve these results significantly. Surveys of the matter distribution are the new frontier for non-Gaussianity, and the SKA has the potential to deliver game-changing constraints, given the ultra-large scales that it probes. This expectation is supported by recent forecasts of the constraining power of different SKA surveys. Another advantage for SKA arises from the possibility of discriminating between different source types, allowing the use of the so-called multi-tracer technique to reduce cosmic variance and thus further increase the constraining capabilities on very large scales. 

Tests of GR on cosmological scales can only be based on a combination of observations of the large-scale structure. Current constraints are weak, but with its huge volumes and multiple probes, the SKA should lead the next generation of tests. In addition, we can strengthen the current tests of dark energy and modified gravity models by including much larger scales, increasing the statistical power of the observations and improving constraints on any scale dependence of deviations from GR.
Probing ultra-large scales includes a theoretical challenge that has only been recently recognized. On very large scales, relativistic effects on the galaxy over-density and the HI brightness temperature fluctuations also become important. They arise since we observe on the past lightcone and they can significantly change the predictions of the standard Newtonian approximation. In addition to the standard redshift-space distortions and the weak lensing magnification, there are Doppler, Sachs-Wolfe, integrated SW and time-delay contributions, which can become significant on horizon scales. It is therefore necessary to include these effects in predictions that will be tested against observations.
The SKA has the potential to detect these relativistic effects, thus providing a clear signal of GR— or an indication of its violation on the largest scales. Furthermore, the amplitude of the relativistic effects can be of the same order as primordial local non-Gaussianity that is consistent with Planck’s constraints. Here we will briefly discuss techniques to improve constraints on primordial non-Gaussianity also taking into account  GR effects.

\subsection{IM cross-correlation}
Cross correlations between HI intensity mapping and optical galaxy surveys can provide precise and robust cosmological measurements, as they have the advantage of mitigating major issues like systematics and foreground contaminants that are relevant for one type of survey but not for the other. For example, in \citet{Masui:2012zc} the intensity maps acquired at the Green Bank telescope were combined with the WiggleZ galaxy survey to constrain the quantity $\Omega_{\rm HI}b_{\rm HI}r$ at $z\sim 0.8$ with a statistical fractional error $\sim 16\%$. 

We will first study cross-correlations with spectroscopic optical galaxy surveys like Euclid, following \citet{Pourtsidou:2016dzn}.
Figure~\ref{fig:PHI}, left, shows the expected signal and  errors for a Euclid-like spectroscopic sample \citep{Majerotto:2012mf} for a redshift bin of width $\Delta z = 0.1$ centered at $z=1$. The assumed sky overlap  is 7,000\,deg$^2$ with corresponding 2,800\,hr total observing time for the IM survey. The resulting constraints on $\Omega_{\rm HI}b_{\rm HI}r$ (keeping the cosmological parameters fixed to the Planck 2015 cosmology \citep{Ade:2015xua}) are summarised in Table~\ref{tab:omHIbHI}. Modifying our approach, we consider $\bar{T}_b$ known and constrain $f\sigma_8$, $D_A$ and $H$.

Cross-correlations with photometric optical galaxy surveys can also be used to constrain HI properties, and perform joint probes studies \citep{Pourtsidou:2015mia}. Figure~\ref{fig:PHI}, right, shows the expected signal and  errors for Stage III (DES-like\footnote{http://www.darkenergysurvey.org/}) photometric sample for a redshift bin of width $\Delta z = 0.1$ centered at $z=0.5$. The assumed sky overlap  is 5,000\,deg$^2$. We can also combine probes such as HI clustering and optical lensing, or HI clustering and the CMB, to constrain gravity \citep{Pourtsidou:2015ksn} and inflation \citep{Pourtsidou:2016ctq}.
An interesting new idea is using HI intensity mapping for photometric redshift calibration. This will be presented in the next section. 

\begin{figure}
\centering
\subfloat{\includegraphics[width=0.5\textwidth]{Synergies/PHIg_zc_1.pdf}}
\subfloat{\includegraphics[width=0.5\textwidth]{Synergies/PHIg-DES.pdf}}
\caption{HI detection in cross-correlation, showing the expected signal power spectrum (black solid) and measurement errors (cyan). {\it Left}: Cross-correlation with a Euclid-like optical galaxy survey. {\it Right}: Cross-correlation with a DES-like optical galaxy survey. The assumed $k$ binning is $\Delta k = 0.01$.}
\label{fig:PHI}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
\caption{\label{tab:omHIbHI} Forecast fractional uncertainties on HI and cosmological parameters assuming the SKA1-MID IM and Euclid-like specifications described in the main text. Note that the assumed redshift bin width is $\Delta z = 0.1$, but we show the results for half of the bins for brevity.}  
\begin{tabular}{ccccc}
\hline
$z$ & $\delta(\Omega_{\rm HI}b_{\rm HI}r)/(\Omega_{\rm HI}b_{\rm HI}r)$
& $\delta(f\sigma_8)/(f\sigma_8)$
& $\delta D_A/D_A$
& $\delta H/H$\\
\hline
1.0&0.019&0.06&0.03&0.02\\
1.2&0.024&0.08&0.05&0.02\\
1.4&0.031&0.10&0.06&0.03\\
1.6&0.039&0.13&0.08&0.03\\
1.8&0.049&0.16&0.1&0.04\\
2.0&0.061&0.19&0.12&0.04\\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Synergies for estimation of redshift distribution of sources}
%Cunnington, Harrison, Pourtsidou, Bacon
With next generation optical surveys such as \textit{Euclid} and LSST promising to deliver unprecedented numbers of resolved galaxies, immense strain will be placed on the amount of spectroscopic follow-up required. Through a clustering-based redshift estimation method which utilities H\,\textsc{i} intensity maps with excellent redshift resolution a well-constrained prediction can be made on the redshift distribution for an arbitrarily large optical population.

SKA intensity mapping would be capable of reducing uncertainties in photometric redshift measurements below the requirements of DES and LSST \cite{Alonso:2017dgh} assuming adequate foreground cleaning could be achieved. Tests have been carried out whereby attempts were made to recover the redshift distribution for an optical galaxy catalogue using simulated H\,\textsc{i} intensity maps (Cunnington et al.(in prep)) built using the S$^3$-SAX catalogue of galaxies \cite{Obreschkow:2009gw}. 

The effects of a foreground clean has been tested in these simulations by removing large radial modes from the data which is the likely impact one would experience from a foreground removal algorithm. This is because most foreground contamination has smoothly fluctuating modes and hence it is  only the small $k_\parallel$ modes in the data that are expected to be inseparable from the foregrounds. We quantify the amount of  $k_\parallel$ modes to remove with the parameter $\xi$ whereby

\begin{equation}\label{kFGmode}
		k^\text{FG}_{\parallel} \approx \frac{\pi H(z)}{c(1+z)\xi}
\end{equation}

and we nullify all modes where $k_\parallel < k^\text{FG}_{\parallel} $. A value of $\xi=0.1$ is considered to be a conservative value for an effective foreground clean \cite{Alonso:2017dgh}.

Figure \ref{ClusteringzdNdz} shows the potential success this method can have and highlights a way that overlapping photometric surveys can benefit from synergies with the SKA.

\begin{figure}
\centering
\subfloat[No Foreground Contamination]{\includegraphics[width=0.5\textwidth]{Synergies/ClusteringzdNdz}}
\subfloat[Simulated Foreground Clean ($\xi=0.1$)]{\includegraphics[width=0.5\textwidth]{Synergies/ClusteringzdNdz_xi01}}
\caption{Testing the feasibility of using H\,\textsc{i} intensity maps to recover the redshift distribution of an optical galaxy catalogue. Results obtained with clustering-based redshift estimation method using intensity maps simulated from S$^3$-SAX catalogue as the reference sample. (a) shows the method assuming no foreground contamination and (b) shows the additional noise one would expect from a foreground clean using a parameter of $\xi=0.1$ outlined in equation \eqref{kFGmode}}
\label{ClusteringzdNdz}
\end{figure}

==> WL/WL.tex <==
\newcommand{\E}{\times10}
\newcommand{\mr}{\mathrm}
\newcommand{\om}{\Omega_\mr m}
\newcommand{\omb}{\Omega_\mr b}
\newcommand{\sig}{\sigma_8}
\newcommand{\pd}{P_{\delta}}
\newcommand{\Clobs}{\widetilde{C}_\ell}
\newcommand{\w}{w_0}
\newcommand{\wa}{w_a}
\newcommand{\cosmosis}{\textsc{CosmoSIS}}
\newcommand{\des}{DES\xspace}
\newcommand{\euclid}{\textit{Euclid}-like}
\newcommand{\planck}{\textit{Planck}}
\renewcommand{\d}{{\rm d}}
Statistical measurement of the shapes of millions of galaxies as a function of sky position and redshift enables us to measure the gravitational lensing effect of all matter, dark and baryonic, along the line of sight between us and those galaxies. Weak lensing shear measurements are insensitive to confounding factors such as galaxy bias, and current surveys are approach the levels of precision in cosmological parameter measurement of other leading probes such as the CMB \cite[e.g.][]{DES, KiDS}. Here, we demonstrate the capabilities of SKA1 as a weak lensing experiment, both alone and in cross-correlation with optical lensing experiments. Here we consider only a total intensity continuum lensing survey, but note that useful information could also be gained on the important intrinsic alignment astrophysical systematic by using polarisation \citep{Brown:2010rr,Brown:2011db,Thomas:2016xhb} and resolved rotational velocity \citep[e.g.][]{Morales:2006fq} measurements.

\subsection{Assumed telescope and survey specifications}
We create forecasts for the Medium-deep survey using SKA1-MID Band 2. This survey is closely analogous to the optimal observing configuration found from catalogue-level simulations in \cite{2016MNRAS.463.3686B}. For comparison to a similar (`DETF Stage III')optical weak lensing experiment, and for use in shear cross-correlations, we take the Dark Energy Survey \citep[DES,][]{} with expectations for the full 5-year survey. Both surveys are fully specified in \cref{tab:experiments}.
\begin{table*}[hb]
\begin{tabular}{lccccccccccc}
\hline 
Experiment & $A_{\rm sky} \, [\mathrm{deg}^2]$ & $n_{\rm gal} \, [\mathrm{arcmin}^{-2}]$ & $z_{m}$ & $\alpha$ & $\beta$ & $\gamma$ & $f_{\textrm{spec-}z}$ & $z_{\textrm{spec-max}}$ & $\sigma_{\textrm{photo-}z}$ & $z_{\textrm{photo-max}}$ & $\sigma_{\textrm{no-}z}$ \\
\hline
SKA1 & 5,000 & 2.7 & 1.1 & $\sqrt{2}$ & 2 & 1.25 & 0.15 & 0.6 & 0.05 & 2.0 & 0.3 \\
\des & 5,000 & 12 & 0.6 & $\sqrt{2}$ & 2 & 1.5 & 0.0 & 2.0 & 0.05 & 2.0 & 0.3 \\
\hline
\end{tabular}
\caption{Parameters used in the creation of simulated data sets for the representative experiments considered in this paper.}
\label{tab:experiments}
\end{table*}
\subsubsection{Redshift information}
We assume redshift distributions for weak lensing galaxies follow a distribution of the form:
\begin{equation}
\label{eqn:nofz}
\frac{\d n_{\rm gal}}{\d z} = z^{\beta} \exp\left( -(z/z_0)^{\gamma} \right),
\end{equation}
where $z_0 = z_{m} / \alpha$ ($\alpha$ is a scale parameter) and $z_{m}$ is the median redshift of sources and with parameters for the SKA1-MID Medium-deep and DES surveys given in \cref{tab:experiments}. Sources are split into ten tomographic redshift bins, with equal numbers of sources in each bin. Sources are also given redshift errors in accordance with the expected information available. A fraction $f_{\textrm{spec-}z}$ out to a redshift of $z_{\textrm{spec-max}}$ are assumed to have spectroscopic errors, in line with the predictions of \cite{bull,harrisonlochner}. The remainder are given photometric redshift errors with a Gaussian distribution (constrained with the physical prior $z>0$) of width $(1+z)\sigma_{\textrm{photo-}z}$ out to a redshift of $z_{\textrm{photo-max}}$. Beyond $z_{\textrm{photo-max}}$ we assume very poor redshift information, with $(1+z)\sigma_{\textrm{no-}z}$.
\subsubsection{Shear measurement}
Of crucial importance to weak lensing cosmology is precise, accurate measurement of source shapes in order to infer the shear transformation resulting from gravitational lensing. For our forecasts, we assume systematic errors due to shear measurement will be sub-dominant to statistical ones. For the Medium-deep survey, the formulae of \cite{2008MNRAS.391..228A} allow us to calculate requirements on the multiplicative shear bias of $\sigma_{m} < 6.4\E^{-3}$ and additive shear bias of $\sigma_{c} < 8.0\E^{-4}$. These requirements are on the same order of magnitude for those achieved in current optical weak lensing surveys such as DES and KiDS, but tighter (by an order of magnitude in the case of multiplicative bias) than current methods for radio interferometer date \citep{2018MNRAS.tmp..362R}. We assume that in the period to 2028, when observations are currently expected to begin, that sufficient progress is made in radio shear measurement methods that biases are comparable to those achievable in optical surveys today. Previous work has shown this is highly unlikely to be possible with images created with the \textsc{CLEAN} algorithm \citep{} meaning access to lower level data products such as gridded visibilities will be essential \citep[see also][]{}. For the intrinsic ellipticity distribution of galaxies we take a shape dispersion of $\sigma_{g_i} = 0.3$, consistent with optical expectations and the findings of \cite{tunbridge}.
\subsection{Forecasting}
We perform our forecasting within the \cosmosis\ cosmological parameter estimation framework \citep{zuntz}. For a given set of cosmological parameters $\boldsymbol\vartheta$ we calculate a non-linear matter power spectrum using CAMB \citep{2000ApJ...538..473L} (with modifications from ISiTGR for the modified gravity models from \citealt{2011PhRvD..84l3001D, 2015PhRvD..92b3003D}) and halofit \citep{2003MNRAS.341.1311S, 2012ApJ...761..152T}. This is then converted to a shear power spectrum using \cref{eqn:limber_cross} and the assumed $n_{X_i}(z)$ for the relevant experiment and redshift bin, including all scales up to $\ell_{\rm max} = 3000$, capturing mildly non-linear scales, dependent on the redshift being probed. The parameter space is explored using the MultiNest algorithm \cite{multinest} to form the contours displayed in \cref{sec:results}, all of which are marginalised over the base \lcdm parameter set $\boldsymbol\vartheta_\lcdm = \lbrace \om, \omb, \sigma_8, h_0, n_s \rbrace$ with the optical depth to reionisation parameter $\tau$ kept fixed.
\subsubsection{Cosmic shear auto-correlations}
The signal of interest, the cosmic shear power spectrum formed from the cross-correlation of shear maps $X_i$ and $Y_j$ (where $X,Y$ are taken to label experiments and $i,j$ redshift bins)is given by:
\begin{equation}
\label{eqn:limber_cross}
C ^{X_{i}Y_{j}} _\ell = \frac{9H_0^4 \om^2}{4c^4} \int_0^{\chi_\mr h} 
\mr d \chi \, \frac{g^{X_i}(\chi) g^{Y_j}(\chi)}{a^2(\chi)} \pd \left(\frac{\ell}{f_K(\chi)},\chi \right) \,,
\end{equation}
where $H_0$ is the Hubble constant, $\om$
is the (total) matter density, $c$ is the speed of light, $a(\chi)$
is the scale factor of the Universe at co-moving distance $\chi$,
$f_K(\chi)$ is the angular diameter distance (given simply by
$f_K(\chi) = \chi$ in a flat Universe), $\pd(k, \chi)$ is the
matter power spectrum and the functions $g^{X_i}(\chi)$ are the lensing
kernels for the redshift bins in question. The lensing kernels are given by:
\begin{equation}
g^{X_i}(\chi) = \int_\chi^{\chi_{\mr h}} \mr d \chi' n_{X_i} (\chi') \frac{f_K (\chi'-\chi)}{f_K (\chi')} \,.
\end{equation}
with respect to the galaxy redshift distributions $n_{i}$ for the relevant experiment and bin. The uncertainty due to shot noise from finite numbers of galaxies sampling the shear field in the measurement of each power spectrum leads to the addition of a noise power spectrum to form the observed:
\begin{equation}
\label{eqn:clobs}
\Clobs^{X_i Y_j} = C_\ell^{X_i Y_j} + \mathcal{N}_\ell^{X_i Y_j},
\end{equation}
which in the case of auto-correlations (i.e. shear spectra using only one experiment) is given by:
\begin{equation}
\label{eqn:autonoise}
\mathcal{N}_\ell^{ij} = \delta^{ij}\frac{\sigma^2_{g_i}}{n^{i}_{\rm gal}}.
\end{equation}

\subsubsection{Cosmic shear cross-correlations}\label{ssec:wl-xcorr}
There are significant advantages to forming cosmic shear power spectra by cross-correlating shear maps made using two different experiments. In such power spectra, wavelength-dependent additive and multiplicative systematics can be removed \cite{Camera:2016owj} and almost all of the statistical constraining power on cosmological parameters is retained \cite{2016MNRAS.463.3674H}.

The use of cross-power spectra necessitates a modification to the noise power spectra \cref{eqn:clobs}. The noise power spectrum is affected by the overlap in shape information between cross-experiment bins $X_i$ and $Y_j$, which is a function of the number of galaxies which have shapes measured by both experiments $n_{\rm gal}^{X_i Y_j}$ and the covariance between their shapes at different wavelengths $\mathrm{cov}(\epsilon_{X_i}, \epsilon_{Y_j}$):
\begin{align}
\mathcal{N}_\ell^{X_i Y_j} &= \frac{1}{n_{\rm gal}^{X_i}n_{\rm gal}^{Y_j}}\langle \sum_{\alpha \in X_i}\epsilon_\alpha  \sum_{\beta \in Y_j}\epsilon_\beta \rangle \nonumber \\
&= \frac{n_{\rm gal}^{X_i Y_j}}{n_{\rm gal}^{X_i}n_{\rm gal}^{Y_j}}\mathrm{cov}(\epsilon_{X_i}, \epsilon_{Y_j}).
\end{align}
Here, we make the simplifying assumption that galaxies have the same shapes and shape variance in both optical wavebands, giving the simplified noise term used in our forecasts:
\begin{equation}
\label{eqn:simplenoise}
\mathcal{N}_\ell^{X_i Y_j} = \frac{n_{\rm gal}^{X_i Y_j}}{n_{\rm gal}^{X_i}n_{\rm gal}^{Y_j}}\sigma^2_{g}.
\end{equation}
We note that constraints are relatively insensitive to the number of galaxies which are present in both bins, being degraded by only $4\%$ when the fraction of overlap is varied between zero and one \citep[see][Fig.~1]{2016MNRAS.463.3674H}.
\subsection{Results}
\label{sec:results}
We show forecast constraints in three cosmological parameter spaces in \cref{fig:wl-shear-forecast}: matter ($\om$-$\sigma_8$), Dark Energy equation of state in the CPL parameterisation ($\w$-$\wa$) and modified gravity modifications to the Poisson equation and Gravitational slip ($\Sigma_0$-$Q_0$). Our results show that the SKA1-Medium-deep survey will be capable of comparable constraints to other DETF Stage III surveys such as DES and also, powerfully, that cross-correlation constraints (which are free of wavelength-dependent systematics) retain almost all of the statistical power as the individual experiments.
\begin{figure}
 \centering
 \includegraphics[width=0.33\columnwidth]{WL/matter.png}
 \includegraphics[width=0.33\columnwidth]{WL/w0wa.png}
  \includegraphics[width=0.33\columnwidth]{WL/mg.png}
 \caption{Forecast constraints for the SKA1-Medium-deep weak lensing survey as specified in the text, compared to the Stage III optical weak lensing Dark Energy Survey (DES) and including cross-correlation constraints.}
 \label{fig:wl-shear-forecast} 
\end{figure}
In \cref{fig:wl-shear-forecast-planck} we also present forecast constraints in the Dark Energy parameter space including priors from the \planck\ CMB experiment, specifically a Gaussian approximation to the \textsc{base-plikHM-TTTEEE-lowTEB-post lensing-BAO} likelihood, with constraints on the other parameters considered not significantly affected by application of the \planck\ prior.
\begin{figure}
 \centering
 \includegraphics[width=0.33\columnwidth]{WL/w0wa_planck.png}
 \caption{The effect of including a prior from the \planck\ satellite on the forecast Dark Energy constraints for the specified cross-correlation survey (note that constraints in the other two parameter spaces on not significantly affected).}
 \label{fig:wl-shear-forecast-planck}
\end{figure}
We also display tabulated summaries of the one dimensional marginalised uncertainties on these parameters in \cref{tab:marginals}.
\begin{table*}[h]
\begin{center}
\begin{tabular}{lrl|rl|rl|c}
\hline 
Experiment & ($\sigma_{\om}/\om$, & $\sigma_{\sigma_{8}}/\sigma_8$) & ($\sigma_{\w}$, & $\sigma_{\wa}$) & ($\sigma_{\Sigma_{0}}/\Sigma_0$, & $\sigma_{Q_{0}}/Q_0$) & DETF FoM\\
\hline
SKA1-Medium-deep & 0.083 & 0.040 & 0.52 & 1.6 & 0.19 & 0.43 & 1.6\\
SKA1-Medium-deep + \planck\ & 0.084 & 0.040 & 0.28 & 0.43 & - & - & 77\\
\des & 0.056 & 0.032 & 0.43 & 1.4 & 0.13 & 0.43 & 3.5\\
\des + \planck\ & 0.058 & 0.033 & 0.22 & 0.33 & - & - & 89\\
SKA1-Medium-deep$\times$\des & 0.046 & 0.024 & 0.45 & 1.3 & 0.13 & 0.39 & 3.3\\
SKA1-Medium-deep$\times$\des + \planck\ & 0.046 & 0.024 & 0.23 & 0.36 & - & - & 106\\
\hline
\end{tabular}
\end{center}
\caption{One dimensional marginalised constraints on the parameters considered, where all pairs (indicated by brackets) are also marginalised over the base \lcdm parameter set.}
\label{tab:marginals}
\end{table*}
